On KL-Regularized Policy Optimization

Asynchronous reinforcement learning (RL) for large language model (LLM) agents trains one policy on trajectories generated by another: rollouts come from stale checkpoints, and the inference engine's probabilities differ from the trainer's even at identical parameters. Standard remedies either clip importance ratios, which biases the update, or, as in GRPO, sample a group of responses per prompt, which is costly when episodes are long. We propose KL-Regularized Policy Optimization (KLPO), a framework that anchors the KL regularizer at the sampler. The regularized improvement step then has a closed-form Gibbs solution, and KLPO fits its log-ratio optimality condition by least squares on the sampler's own trajectories, so the sampler probability enters through a log-ratio and no importance weights are needed. Profiling out the regression intercept replaces the intractable log-partition function with the signal's sampler mean plus a sampler-to-trainer KL divergence. For token-level policy mirror descent targets, we show that the resulting gradient can be computed from terminal returns without a critic, via sampler-centered scores or a single trajectory residual, even under stochastic tool outputs. We further prove that independent Monte Carlo estimates of the KL term keep these gradients unbiased, derive the exact KL gap of cheaper top-$K$ and binary approximations, and show that SPPO, GPO, REBEL, and BPO arise as special cases of KLPO. The result is a critic-free update that uses one rollout per prompt and requires neither a learned normalizer nor a group of responses.

==> figures/style.tex <==
% Figure-local palette inspired by the RLT manuscript; no document theme changes.
\definecolor{klpoInk}{HTML}{172B4D}
\definecolor{klpoBlue}{HTML}{007AFF}
\definecolor{klpoOrange}{HTML}{E87500}
\definecolor{klpoGray}{HTML}{667085}
\definecolor{klpoLine}{HTML}{DCE3EB}
\tikzset{
 klpo box/.style={rounded corners=3pt,draw=klpoBlue!55,fill=white,
   text=klpoInk,align=center,inner sep=5pt,minimum height=.65cm},
 klpo fit/.style={klpo box,draw=klpoOrange!65,fill=klpoOrange!5},
 klpo flow/.style={->,draw=klpoBlue,line width=.85pt},
 klpo update/.style={->,draw=klpoOrange,line width=1.15pt},
 klpo note/.style={font=\sffamily\footnotesize,text=klpoGray},
 klpo heading/.style={font=\sffamily\bfseries,text=klpoInk,anchor=west}
}

